Sok: Comprehensive Security Overview, Challenges, and Future Directions of Voice-Controlled Systems

The integration of Voice Control Systems (VCS) into smart devices and their growing presence in daily life accentuate the importance of their security. Current research has uncovered numerous vulnerabilities in VCS, presenting significant risks to user privacy and security. However, a cohesive and systematic examination of these vulnerabilities and the corresponding solutions is still absent. This lack of comprehensive analysis presents a challenge for VCS designers in fully understanding and mitigating the security issues within these systems. Addressing this gap, our study introduces a hierarchical model structure for VCS, providing a novel lens for categorizing and analyzing existing literature in a systematic manner. We classify attacks based on their technical principles and thoroughly evaluate various attributes, such as their methods, targets, vectors, and behaviors. Furthermore, we consolidate and assess the defense mechanisms proposed in current research, offering actionable recommendations for enhancing VCS security. Our work makes a significant contribution by simplifying the complexity inherent in VCS security, aiding designers in effectively identifying and countering potential threats, and setting a foundation for future advancements in VCS security research.

==> body/abstract.tex <==
\begin{abstract}
The integration of Voice Control Systems (VCS) into smart devices and their growing presence in daily life accentuate the importance of their security. 
Current research has uncovered numerous vulnerabilities in VCS, presenting significant risks to user privacy and security. 
However, a cohesive and systematic examination of these vulnerabilities and the corresponding solutions is still absent. 
This lack of comprehensive analysis presents a challenge for VCS designers in fully understanding and mitigating the security issues within these systems.

Addressing this gap, our study introduces a hierarchical model structure for VCS, 
providing a novel lens for categorizing and analyzing existing literature in a systematic manner. 
We classify attacks based on their technical principles and thoroughly evaluate various attributes, 
such as their methods, targets, vectors, and behaviors. 
Furthermore, we consolidate and assess the defense mechanisms proposed in current research, 
offering actionable recommendations for enhancing VCS security. 
Our work makes a significant contribution by simplifying the complexity inherent in VCS security, 
aiding designers in effectively identifying and countering potential threats, and setting a foundation for future advancements in VCS security research.




    
\end{abstract}

==> body/attack.tex <==
\section{Attack against Voice-}


We begin by identifying the attack surface of ML systems to inform where and how an adversary will attempt to
subvert the system. Our development of the threat model in



\subsection{}
\subsubsection{Voice replay attack (VRA)}

\subsubsection{Voice conversion attack (VCA)}


\subsection{Adversarial audio examples (AAE)}

\subsection{}
